Component Analysis for Visual Question Answering Architectures

Recent research advances in Computer Vision and Natural Language Processing have introduced novel tasks that are paving the way for solving AI-complete problems. One of those tasks is called Visual Question Answering (VQA). A VQA system must take an image and a free-form, open-ended natural language question about the image, and produce a natural language answer as the output. Such a task has drawn great attention from the scientific community, which generated a plethora of approaches that aim to improve the VQA predictive accuracy. Most of them comprise three major components: (i) independent representation learning of images and questions; (ii) feature fusion so the model can use information from both sources to answer visual questions; and (iii) the generation of the correct answer in natural language. With so many approaches being recently introduced, it became unclear the real contribution of each component for the ultimate performance of the model. The main goal of this paper is to provide a comprehensive analysis regarding the impact of each component in VQA models. Our extensive set of experiments cover both visual and textual elements, as well as the combination of these representations in form of fusion and attention mechanisms. Our major contribution is to identify core components for training VQA models so as to maximize their predictive performance.

==> README <==

January 11, 2007


IEEEtran.bst is the official BibTeX style for authors of the Institute of
Electrical and Electronics Engineers (IEEE) Transactions journals and
conferences.

It also may have applications for other academic work such as theses and
technical reports. The alphanumeric and natbib variants extend the
applicability of the IEEEtran bibstyle family to the natural sciences
and beyond.

The IEEEtran bibstyle is a very comprehensive BibTeX style which provides
many features beyond the standard BibTeX styles, including full support
for references of online documents, patents, periodicals and standards.
See the provided user manual for detailed usage information.

The latest version of the IEEEtran BibTeX style can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/bibtex/

as well as within IEEE's site:

http://www.ieee.org/

Note that the packages at IEEE's site do not contain the natbib and
alphanumeric variants (e.g., IEEEtranN.bst, etc.) as these are not used
for IEEE related work. These files can be obtained on CTAN.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtran home page at my website:

http://www.michaelshell.org/tex/ieeetran/


Enjoy!

Michael Shell
http://www.michaelshell.org/

*******
Version 1.12 (2007/01/11) changes:

 1. Fixed bug with unwanted comma before "et al." when an entry contained
    more than two author names. Thanks to Pallav Gupta for reporting this.

 2. Fixed bug with anomalous closing quote in tech reports that have a
    type, but without a number or address. Thanks to Mehrdad Mirreza for
    reporting this.

 3. Use braces in \providecommand in begin.bib to better support
    latex2html. TeX style length assignments OK with recent versions
    of latex2html - 1.71 (2002/2/1) or later is strongly recommended.
    Use of the language field still causes trouble with latex2html.
    Thanks to Federico Beffa for reporting this.

 4. Added IEEEtran.bst ID and version comment string to .bbl output.

 5. Provide a \BIBdecl hook that allows the user to execute commands
    just prior to the first entry.

 6. Use default urlstyle (is using url.sty) of "same" rather than rm to
    better work with a wider variety of bibliography styles.

 7. Changed month abbreviations from Sept., July and June to Sep., Jul.,
    and Jun., respectively, as IEEE now does. Thanks to Moritz Borgmann
    for reporting this.

 8. Control entry types should not be considered when calculating longest
    label width.

 9. Added alias www for electronic/online.

10. Updated full and abbreviated journal name string definitions in
    IEEEfull.bib and IEEEabrv.bib.

11. New IEEEtranSA.bst, IEEEtranN.bst, and IEEEtranSN.bst variants for
    alphanumeric citation tags and natbib compatibility.


********************************** Files **********************************

README                 - This file.

IEEEtran_bst_HOWTO.pdf - The user manual.

IEEEtran.bst           - The standard IEEEtran BibTeX style file. For use
                         with IEEE work.

IEEEtranS.bst          - A version of IEEEtran.bst that sorts the entries.
                         Some IEEE conferences/publications may use/allow
                         sorted bibliographies.

IEEEexample.bib        - An example BibTeX database that contains the
                         references shown in the user manual.

IEEEabrv.bib           - String definitions for the abbreviated names of
                         IEEE journals. (For use with IEEE work.)
                         
IEEEfull.bib           - String definitions for the full names of IEEE
                         journals. (Do not use for IEEE work.)


Carried on CTAN only, for non-IEEE related work:

IEEEtranSA.bst         - Like IEEEtranS.bst, but with alphanumeric citation
                         tags like alpha.bst. Not for normal IEEE use.

EEEtranN.bst          - Like IEEEtran.bst, but based on plainnat.bst and
                         is compatible with Patrick W. Daly's natbib
                         package. Not for normal IEEE use.

IEEEtranSN.bst         - Sorting version of IEEEtranN.bst. Not for normal
                         IEEE use

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran_bst_HOWTO.pdf, IEEEtran.bst, IEEEtranS.bst,
                   IEEEtranSA.bst, IEEEtranN.bst, IEEEtranSN.bst,
                   IEEEexample.bib, IEEEabrv.bib, IEEEfull.bib
                   
***************************************************************************


==> VQA%20Component%20Analysis%20(IJCNN%202020)/README <==

January 11, 2007


IEEEtran.bst is the official BibTeX style for authors of the Institute of
Electrical and Electronics Engineers (IEEE) Transactions journals and
conferences.

It also may have applications for other academic work such as theses and
technical reports. The alphanumeric and natbib variants extend the
applicability of the IEEEtran bibstyle family to the natural sciences
and beyond.

The IEEEtran bibstyle is a very comprehensive BibTeX style which provides
many features beyond the standard BibTeX styles, including full support
for references of online documents, patents, periodicals and standards.
See the provided user manual for detailed usage information.

The latest version of the IEEEtran BibTeX style can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/bibtex/

as well as within IEEE's site:

http://www.ieee.org/

Note that the packages at IEEE's site do not contain the natbib and
alphanumeric variants (e.g., IEEEtranN.bst, etc.) as these are not used
for IEEE related work. These files can be obtained on CTAN.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtran home page at my website:

http://www.michaelshell.org/tex/ieeetran/


Enjoy!

Michael Shell
http://www.michaelshell.org/

*******
Version 1.12 (2007/01/11) changes:

 1. Fixed bug with unwanted comma before "et al." when an entry contained
    more than two author names. Thanks to Pallav Gupta for reporting this.

 2. Fixed bug with anomalous closing quote in tech reports that have a
    type, but without a number or address. Thanks to Mehrdad Mirreza for
    reporting this.

 3. Use braces in \providecommand in begin.bib to better support
    latex2html. TeX style length assignments OK with recent versions
    of latex2html - 1.71 (2002/2/1) or later is strongly recommended.
    Use of the language field still causes trouble with latex2html.
    Thanks to Federico Beffa for reporting this.

 4. Added IEEEtran.bst ID and version comment string to .bbl output.

 5. Provide a \BIBdecl hook that allows the user to execute commands
    just prior to the first entry.

 6. Use default urlstyle (is using url.sty) of "same" rather than rm to
    better work with a wider variety of bibliography styles.

 7. Changed month abbreviations from Sept., July and June to Sep., Jul.,
    and Jun., respectively, as IEEE now does. Thanks to Moritz Borgmann
    for reporting this.

 8. Control entry types should not be considered when calculating longest
    label width.

 9. Added alias www for electronic/online.

10. Updated full and abbreviated journal name string definitions in
    IEEEfull.bib and IEEEabrv.bib.

11. New IEEEtranSA.bst, IEEEtranN.bst, and IEEEtranSN.bst variants for
    alphanumeric citation tags and natbib compatibility.


********************************** Files **********************************

README                 - This file.

IEEEtran_bst_HOWTO.pdf - The user manual.

IEEEtran.bst           - The standard IEEEtran BibTeX style file. For use
                         with IEEE work.

IEEEtranS.bst          - A version of IEEEtran.bst that sorts the entries.
                         Some IEEE conferences/publications may use/allow
                         sorted bibliographies.

IEEEexample.bib        - An example BibTeX database that contains the
                         references shown in the user manual.

IEEEabrv.bib           - String definitions for the abbreviated names of
                         IEEE journals. (For use with IEEE work.)
                         
IEEEfull.bib           - String definitions for the full names of IEEE
                         journals. (Do not use for IEEE work.)


Carried on CTAN only, for non-IEEE related work:

IEEEtranSA.bst         - Like IEEEtranS.bst, but with alphanumeric citation
                         tags like alpha.bst. Not for normal IEEE use.

EEEtranN.bst          - Like IEEEtran.bst, but based on plainnat.bst and
                         is compatible with Patrick W. Daly's natbib
                         package. Not for normal IEEE use.

IEEEtranSN.bst         - Sorting version of IEEEtranN.bst. Not for normal
                         IEEE use

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran_bst_HOWTO.pdf, IEEEtran.bst, IEEEtranS.bst,
                   IEEEtranSA.bst, IEEEtranN.bst, IEEEtranSN.bst,
                   IEEEexample.bib, IEEEabrv.bib, IEEEfull.bib
                   
***************************************************************************


==> VQA%20Component%20Analysis%20(IJCNN%202020)/tables/attention.tex <==

% \begin{table}
% \centering
% \caption{Experiment using different attention mechanisms.}
%     \begin{tabular}{|c|c|c|}
%         \hline
%         Attention & Training & Validation\\
%         \hline
%         No attention & 78.20 & 58.75 \\
%         % \cline{3-7}
%         Top Down & 82.64 & 62.37\\
%         Top Down (block) & 87.02 & \textbf{64.12}\\
%         % \cline{3-7}
%         CoAtt & 71.10 & 58.54\\
%         Stacked & 86.03 & 64.03\\
%         \hline
%     \end{tabular}
%     \label{tab:result_att}
% \end{table}


\begin{table}[!b]
\centering
\caption{Experiment using different attention mechanisms.}
    \begin{tabular}{|c|c|c|c|c|}
        \hline
        \textit{Embedding} & RNN & Attention & Training & Validation \\
        \hline
        \multirow{5}{2em}{BERT} & \multirow{5}{2em}{GRU} & - & 78.20 & 58.75 \\
        & & Co-Attention & 71.10 & 58.54\\
        & & Co-Attention (L2 norm) & 86.03 & 64.03\\
        & & Top Down & 82.64 & 62.37\\
        & & Top Down ($\sigma=$ReLU) & 87.02 & \textbf{64.12}\\
        \hline
    \end{tabular}
    \label{tab:result_att}
\end{table}


==> VQA%20Component%20Analysis%20(IJCNN%202020)/tables/bestmodel.tex <==

\begin{table}
\centering
\caption{Best model per experiment.}
    \begin{tabular}{|c|c|c|c|}
        \hline
        Section & Method & Overall Acc Train & Overall Acc Val\\
        \hline
        - & Original Arch & 82.52 & 56.33 \\
        % \multirow{2}{1em}{\ref{sec:txt_enc}} & BERT-GRU-1HL-4096 & 78,28 & 58,75\\
        % \multirow{2}{1em}{\ref{sec:txt_enc}} & BERT-GRU & 78,28 & 58,75\\
        \ref{sec:txt_enc} & BERT-GRU & 78.28 & 58.75\\
        
        % & SKIP-LSTM-2HL-2048HS & 83,38 & 57,57 \\
        
        \ref{sec:img_enc} & Faster-RCNN & 78.28 & 58.75\\
        
        \ref{sec:fus} & MULT & 78.28 & 58.75 \\ 
        
        \ref{sec:att} & TOP-DOWN & 82.64 & 62.37\\ 
        \hline
        Best Model & - & 82.64 & \textbf{62.37}\\ 
        \hline
    \end{tabular}
    \label{tab:result_summary}
\end{table}


==> VQA%20Component%20Analysis%20(IJCNN%202020)/tables/fusion.tex <==

\begin{table}[!b]
\centering
\caption{Experiment using different fusion strategies.}
    \begin{tabular}{|c|c|c|c|c|c|}
        \hline
        \textit{Embedding} & RNN & Fusion & Training & Validation \\
        \hline
        \multirow{3}{3em}{BERT} & \multirow{3}{2em}{GRU} & Mult & 78.28 & \textbf{58.75} \\ 
        % \cline{3-7}
        & & Concat & 67.85 & 55.07\\ 
        % \cline{3-7}
        & & Sum & 68.21 & 54.93\\ 
        \hline
    \end{tabular}
    \label{tab:result_fusion}
\end{table}

==> VQA%20Component%20Analysis%20(IJCNN%202020)/tables/testset1.tex <==

\begin{table}[!htpb]
\centering
\caption{Comparison of the models on VQA2 test-dev set. \textit{All} is the overall OpenEnded accuracy (higher is better). \textit{Yes/No}, \textit{Numbers}, and \textit{Others} are subsets that correspond to answers types. * scores reported from \cite{ben2019block}.}
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
        \hline
        \multirow{2}{6em}{Model} & \multicolumn{4}{c|}{VQA2.0 Test-Dev} \\
        \cline{2-5}
        & All & Yes/No & Num. & Other \\
        \hline
        \baseline~\cite{antol2015vqa} & 51.95 & 70.42 & 32.28 & 40.64 \\
        MCB* \cite{fukui2016multimodal} & 61.23 & 79.73 & 39.13 & 50.45 \\
        \block*~\cite{ben2019block} & 66.41 & 82.86 & 44.76 & 57.30 \\
        \hline
        % \stbestmodel & 64.03 & 81.87 & 42.73 & 53.65 \\
        BERT-GRU-Faster-CoAttention & 65.84 & 83.66 & 44.36 & 55.50\\
        BERT-GRU-Faster-TopDown & 66.02 & 83.72 & 44.88 & 55.77  \\
        \hline
    \end{tabular}
    \label{tab:sota_comp_vqadev}
\end{table}

% todo RUN WITH VG
% \begin{table*}[t]
% \centering
% \caption{Test-dev and test-std using only vqa 2.0}
%     \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
%         \hline
%         \multirow{2}{6em}{Model} & \multicolumn{4}{c|}{VQA2.0 Test-Dev} & \multicolumn{4}{c|}{VQA2.0 Test-Std}\\
%         \cline{2-9}
%         & All & Yes/No & Num. & Other & All & Yes/No & Num. & Other \\
%         \hline
%         \baseline & 51,75 & 71,74 & 33,77 & 40,82 & 52,99 & 71,76 & 33,35 & 41,14 \\
%         \stbestmodel & 64,03 & 81,87 & 42,73 & 53,65 & 64,44 & 82,39 & 42,44 & 53,86 \\
%         BERT-GRU-FASTER-BLOCKATT & - & - & - & - & - & - & - & - \\
%         \block & 67,58 & 83,60 & 47,33 & 58,51 & 67,92 & 83,98 & 46,77 & 58,79 \\
%         \hline
%     \end{tabular}
%     \label{tab:sota_comp}
% \end{table*}


==> VQA%20Component%20Analysis%20(IJCNN%202020)/tables/text_enc_freeze.tex <==
\begin{table}
\centering
\caption{Results using frozen pre-trained embeddings.}
    \begin{tabular}{|c|c|c|c|}
        \hline
        \textit{Embedding} & RNN & Overall Acc Train & Overall Acc Val\\
        \hline

        \multirow{5}{6em}{Skip Thoughts} & Linear & 77.08 & 54.14 \\ 
        & LSTM & 85.89 & \textbf{57.06} \\ 
        & LSTM Bidir & 85.73 & 57.00 \\ 
        & GRU & 85.97 & 56.96\\
        & GRU (skip) & 82.55 & 55.02\\
        & GRU Bidir & 86.66 & 56.96\\
        \hline

        \multirow{5}{5em}{BERT} & Linear & 59.83 & 49.18\\ 
        & LSTM & 72.96 & 55.06\\ 
        & LSTM Bidir & 72.95 & \textbf{55.18}\\ 
        & GRU & 71.84 & 54.75\\
        & GRU Bidir & 72.38 & 54.88\\
        \hline
        
        \multirow{5}{5em}{GloVe} & Linear & 76.12 & 53.37\\ 
        & LSTM & 86.24 & \textbf{57.20}\\ 
        & LSTM Bidir & 86.86 & 57.08\\ 
        & GRU & 85.67 & 57.12\\
        & GRU Bidir & 86.56 & 57.13\\
        \hline
        
        \multirow{5}{5em}{W2V} & Linear & 75.94 & 53.63\\ 
        & LSTM & 84.33 & 56.87\\ 
        & LSTM Bidir & 84.16 & 56.95\\ 
        & GRU & 84.55 & \textbf{57.05}\\
        & GRU Bidir & 85.33 & 56.92\\
        \hline
        
    \end{tabular}
    \label{tab:result_txtenc_frozenweights}
\end{table}


==> VQA%20Component%20Analysis%20(IJCNN%202020)/tables/text_enc_update.tex <==
    \begin{table}
    \caption{Results using pre-trained embeddings training in conjunction with the model.}
    \centering
        \begin{tabular}{|c|c|c|c|}
            \hline
            \textit{Embedding} & RNN & Overall Acc Train & Overall Acc Val\\
            
            \hline
            \multirow{5}{6em}{\method} & Linear & 78.33 & 54.85 \\ 
            & LSTM & 82.51 & 56.33 \\ 
            & LSTM Bidir & 82.55 & 56.02\\ 
            & GRU & 85.52 & 56.40\\
            & GRU Bidir & 85.70 & \textbf{56.44}\\
            
            \hline
            \multirow{5}{6em}{Skip Thoughts} & Linear & 80.34 & 55.22 \\ 
            & LSTM & 86.84 & \textbf{57.44} \\ 
            & LSTM Bidir & 86.61 & 57.22\\ 
            & GRU & 86.79 & 57.19\\
            & GRU (skip) & 89.25 & 57.06\\
            & GRU Bidir & 87.38 & 57.26\\
            \hline
    
            % \multirow{5}{5em}{BERT} & Linear & 28,24 & 24,24\\ 
            % & LSTM & 32,91 & 23,99 \\ 
            % & LSTM Bidir & 32,96 & 23,94\\ 
            % & GRU & 33,11 & 23,94\\
            % & GRU Bidir & 32,36 & 24,19\\
            % \hline
            \multirow{5}{5em}{BERT} & Linear & 76.59 & 58.28\\ 
            & LSTM & 77.23 & 58.73\\ 
            & LSTM Bidir & 77.05 & 58.73\\ 
            & GRU & 78.28 & \textbf{58.75}\\
            & GRU Bidir & 77.79 & 58.62\\
            \hline
            
            \multirow{5}{5em}{GloVe} & Linear & 78.75 & 55.05\\ 
            & LSTM & 87.17 & 57.28\\ 
            & LSTM Bidir & 87.13 & 57.37\\ 
            & GRU & 85.85 & 57.38\\
            & GRU Bidir & 86.79 & \textbf{57.42}\\
            \hline
            
            \multirow{5}{5em}{W2V} & Linear & 79.23 & 55.36\\ 
            & LSTM & 84.96 & 57.31\\ 
            & LSTM Bidir & 84.94 & 57.34\\ 
            & GRU & 85.32 & 57.30\\
            & GRU Bidir & 86.02 & \textbf{57.39}\\
            \hline
        \end{tabular}
        \label{tab:result_txtenc}
        % \caption*{FONTE: elaborado pelo autor.}
    \end{table}


==> tables/bestmodel.tex <==

\begin{table}
\centering
\caption{Best model per experiment.}
    \begin{tabular}{|c|c|c|c|}
        \hline
        Section & Method & Overall Acc Train & Overall Acc Val\\
        \hline
        - & Original Arch & 82.52 & 56.33 \\
        % \multirow{2}{1em}{\ref{sec:txt_enc}} & BERT-GRU-1HL-4096 & 78,28 & 58,75\\
        % \multirow{2}{1em}{\ref{sec:txt_enc}} & BERT-GRU & 78,28 & 58,75\\
        \ref{sec:txt_enc} & BERT-GRU & 78.28 & 58.75\\
        
        % & SKIP-LSTM-2HL-2048HS & 83,38 & 57,57 \\
        
        \ref{sec:img_enc} & Faster-RCNN & 78.28 & 58.75\\
        
        \ref{sec:fus} & MULT & 78.28 & 58.75 \\ 
        
        \ref{sec:att} & TOP-DOWN & 82.64 & 62.37\\ 
        \hline
        Best Model & - & 82.64 & \textbf{62.37}\\ 
        \hline
    \end{tabular}
    \label{tab:result_summary}
\end{table}


==> tables/text_enc_freeze.tex <==
\begin{table}
\centering
\caption{Results using frozen pre-trained embeddings.}
    \begin{tabular}{|c|c|c|c|}
        \hline
        \textit{Embedding} & RNN & Overall Acc Train & Overall Acc Val\\
        \hline

        \multirow{5}{6em}{Skip Thoughts} & Linear & 77.08 & 54.14 \\ 
        & LSTM & 85.89 & \textbf{57.06} \\ 
        & LSTM Bidir & 85.73 & 57.00 \\ 
        & GRU & 85.97 & 56.96\\
        & GRU (skip) & 82.55 & 55.02\\
        & GRU Bidir & 86.66 & 56.96\\
        \hline

        \multirow{5}{5em}{BERT} & Linear & 59.83 & 49.18\\ 
        & LSTM & 72.96 & 55.06\\ 
        & LSTM Bidir & 72.95 & \textbf{55.18}\\ 
        & GRU & 71.84 & 54.75\\
        & GRU Bidir & 72.38 & 54.88\\
        \hline
        
        \multirow{5}{5em}{GloVe} & Linear & 76.12 & 53.37\\ 
        & LSTM & 86.24 & \textbf{57.20}\\ 
        & LSTM Bidir & 86.86 & 57.08\\ 
        & GRU & 85.67 & 57.12\\
        & GRU Bidir & 86.56 & 57.13\\
        \hline
        
        \multirow{5}{5em}{W2V} & Linear & 75.94 & 53.63\\ 
        & LSTM & 84.33 & 56.87\\ 
        & LSTM Bidir & 84.16 & 56.95\\ 
        & GRU & 84.55 & \textbf{57.05}\\
        & GRU Bidir & 85.33 & 56.92\\
        \hline
        
    \end{tabular}
    \label{tab:result_txtenc_frozenweights}
\end{table}


==> tables/text_enc_update.tex <==
    \begin{table}
    \caption{Results using pre-trained embeddings training in conjunction with the model.}
    \centering
        \begin{tabular}{|c|c|c|c|}
            \hline
            \textit{Embedding} & RNN & Overall Acc Train & Overall Acc Val\\
            
            \hline
            \multirow{5}{6em}{\method} & Linear & 78.33 & 54.85 \\ 
            & LSTM & 82.51 & 56.33 \\ 
            & LSTM Bidir & 82.55 & 56.02\\ 
            & GRU & 85.52 & 56.40\\
            & GRU Bidir & 85.70 & \textbf{56.44}\\
            
            \hline
            \multirow{5}{6em}{Skip Thoughts} & Linear & 80.34 & 55.22 \\ 
            & LSTM & 86.84 & \textbf{57.44} \\ 
            & LSTM Bidir & 86.61 & 57.22\\ 
            & GRU & 86.79 & 57.19\\
            & GRU (skip) & 89.25 & 57.06\\
            & GRU Bidir & 87.38 & 57.26\\
            \hline
    
            % \multirow{5}{5em}{BERT} & Linear & 28,24 & 24,24\\ 
            % & LSTM & 32,91 & 23,99 \\ 
            % & LSTM Bidir & 32,96 & 23,94\\ 
            % & GRU & 33,11 & 23,94\\
            % & GRU Bidir & 32,36 & 24,19\\
            % \hline
            \multirow{5}{5em}{BERT} & Linear & 76.59 & 58.28\\ 
            & LSTM & 77.23 & 58.73\\ 
            & LSTM Bidir & 77.05 & 58.73\\ 
            & GRU & 78.28 & \textbf{58.75}\\
            & GRU Bidir & 77.79 & 58.62\\
            \hline
            
            \multirow{5}{5em}{GloVe} & Linear & 78.75 & 55.05\\ 
            & LSTM & 87.17 & 57.28\\ 
            & LSTM Bidir & 87.13 & 57.37\\ 
            & GRU & 85.85 & 57.38\\
            & GRU Bidir & 86.79 & \textbf{57.42}\\
            \hline
            
            \multirow{5}{5em}{W2V} & Linear & 79.23 & 55.36\\ 
            & LSTM & 84.96 & 57.31\\ 
            & LSTM Bidir & 84.94 & 57.34\\ 
            & GRU & 85.32 & 57.30\\
            & GRU Bidir & 86.02 & \textbf{57.39}\\
            \hline
        \end{tabular}
        \label{tab:result_txtenc}
        % \caption*{FONTE: elaborado pelo autor.}
    \end{table}

